Approximating Optimal Transport via Low-rank and Sparse Factorization

Optimal transport (OT) naturally arises in a wide range of machine learning applications but may often become the computational bottleneck. Recently, one line of works propose to solve OT approximately by searching the \emph{transport plan} in a low-rank subspace. However, the optimal transport plan is often not low-rank, which tends to yield large approximation errors. For example, when Monge's \emph{transport map} exists, the transport plan is full rank. This paper concerns the computation of the OT distance with adequate accuracy and efficiency. A novel approximation for OT is proposed, in which the transport plan can be decomposed into the sum of a low-rank matrix and a sparse one. We theoretically analyze the approximation error. An augmented Lagrangian method is then designed to efficiently calculate the transport plan.

==> sections/methodology_D.tex <==
We first define the approximated distance which decomposes the transport plan into a low-rank matrix and a sparse one.
Next, we derive an augmented Lagrangian method for calculating the proposed distance.
Finally, we analyze the overall complexity of the proposed method.

\subsection{Approximated Distance}
The proposed approximation of OT distance is
\begin{equation}\label{eq:formuation}
	\LSOT_{r,k}(\pB,\qB)=\min_{\AB,\BB,\SB\in\tilde\Omega_{r,k}(\pB,\qB)}\langle \CB,\AB\BB^\top+\SB\rangle,
\end{equation}
where the feasible domain is defined as
\begin{equation*}
	\begin{aligned}
		\tilde\Omega_{r,k}(\pB,\qB)=\Big\{\AB\in\RBB^{m\times r},\BB\in\RBB^{n\times r},\SB\in\RBB^{m\times n}&\Big|0\le\AB\le 1,0\le\BB\le 1,\|\SB\|_0\le k,\\
		&\AB\BB^\top+\SB\ge 0,(\AB\BB^\top+\SB)\oneB=\pB,(\AB\BB^\top+\SB)^\top\oneB=\qB\Big\},
	\end{aligned}
\end{equation*}
and $r\ll\min\{m,n\}$.
By the property of the matrix rank, matrix $\AB\BB^\top$ is low-rank, i.e., $\rank(\AB\BB^\top)\le r\ll\min\{m,n\}$.
$k$ controls the sparsity and satisfies $0\le k\ll mn$.
$\LSOT_{r,k}(\pB,\qB)$ approximates $\OT(\pB,\qB)$ better than $\LOT_{r}(\pB,\qB)$, which is formalized in the following proposition.
\begin{proposition}
	For $0\le r\le\min\{m,n\}$ and $0\le k\le mn$, $\OT(\pB,\qB)\le \LSOT_{r,k}(\pB,\qB)\le \LOT_{r}(\pB,\qB)$. When either
	\begin{equation*}
		r\ge\min_{\TB^*\in\argmin_\TB\langle\CB,\TB\rangle}\rankp(\TB^*),
	\end{equation*}
	 or $k\ge m+n-1$ holds, $\OT(\pB,\qB)= \LSOT_{r,k}(\pB,\qB)$.
\end{proposition}
The proof is deferred to the appendix.
It is difficult to determine the \nonnegative{} rank of an optimal transport plan \citep{cohen1993nonnegative}.
However, $\OT(\pB,\qB)$ can be recovered with $k\ge m+n-1$.

\subsection{Optimization}

\paragraph{Surrogate problem.}
The $\|\SB\|_0\le k$ constraint in $\tilde\Omega_{r,k}(\pB,\qB)$ makes problem (\ref{eq:formuation}) intractable.
%We thus consider the following surrogate problem
%\begin{equation}\label{eq:surrogate}
%	\min_{\AB,\BB,\SB\in\Omega_{r,k}(\pB,\qB)}\langle \CB,\AB\BB^\top+\SB\rangle+\lambda\|\SB\|_1,
%\end{equation}
%where the feasible domain is given by
%\begin{equation*}
%	\begin{aligned}
%		\Omega_{r,k}(\pB,\qB)=\Big\{\AB\in\RBB^{m\times r},\BB\in\RBB^{n\times r},\SB\in\RBB^{m\times n}&\Big|0\le\AB\le 1,0\le\BB\le 1,\\
%		&\AB\BB^\top+\SB\ge 0,(\AB\BB^\top+\SB)\oneB=\pB,(\AB\BB^\top+\SB)^\top\oneB=\qB\Big\}.
%	\end{aligned}
%\end{equation*}
We thus consider the following surrogate problem
\begin{equation}\label{eq:surrogate}
	\min_{\AB,\BB,\SB,\DB\in\Omega_{r,k}(\pB,\qB)}\langle \CB,\AB\BB^\top+\SB\rangle+\lambda\|\SB\|_1,
\end{equation}
where the feasible domain is given by
\begin{equation*}
	\begin{aligned}
		\Omega_{r,k}(\pB,\qB)=\Big\{\AB\in\RBB^{m\times r},\BB\in\RBB^{n\times r},\SB\in\RBB^{m\times n},\DB\in\RBB^{m\times n}&\Big|0\le\AB\le 1,0\le\BB\le 1,\DB\ge0,\\
		&\AB\BB^\top+\SB=\DB,(\AB\BB^\top+\SB)\oneB=\pB,(\AB\BB^\top+\SB)^\top\oneB=\qB\Big\}.
	\end{aligned}
\end{equation*}
Note that the inequality constraint $\AB\BB^\top+\SB\ge0$ has been converted into an equality constraint $\AB\BB^\top+\SB=\DB$ by enforcing the \nonnegativity{} of $\DB$.
Because of the \bilinear{} terms, (\ref{eq:surrogate}) has a \nonconvex{} objective function and \nonconvex{} constraints.
Stationary points can be found effectively by an inexact augmented Lagrangian method (ALM).



\paragraph{Inexact ALM.}
ALM is a classical algorithm for constrained optimization \citep{hestenes1969multiplier,powell1969method}.
For solving (\ref{eq:surrogate}), ALM suggests solving
\begin{equation}\label{eq:problem_alm}
	\min_{\AB,\BB,\SB,\DB}\max_{\yp,\yq,\yd}\lag(\AB,\BB,\SB,\DB,\yp,\yq,\yd,\beta)+\lambda\|\SB\|_1+\ia(\AB)+\ib(\BB)+\id(\DB),
\end{equation}
where $\ia(\cdot)$, $\ib(\cdot)$ and $\id(\cdot)$ are indicator functions corresponding to $0\le\AB\le 1$, $0\le\BB\le 1$, and $\DB\ge 0$ respectively.
The augmented Lagrangian function is defined as
\begin{equation}
	\begin{aligned}
		\lag(\AB,\BB,\SB,\DB,\yp,\yq,\yd,\beta)&=\langle\CB,\AB\BB^\top+\SB\rangle+\frac{\beta}{2}\Big(\|(\AB\BB^\top+\SB)\oneB-\pB\|^2+\|(\AB\BB^\top+\SB)^\top\oneB-\qB\|^2+\|\AB\BB^\top+\SB-\DB\|^2_F\Big)\\
		&+\langle \yp,(\AB\BB^\top+\SB)\oneB-\pB\rangle+\langle \yq,(\AB\BB^\top+\SB)^\top\oneB-\qB\rangle+\langle \yd, \AB\BB^\top+\SB-\DB\rangle,
	\end{aligned}
\end{equation}
where $\yp\in\RBB^m$, $\yq\in\RBB^n$, and $\yd\in\RBB^{m\times n}$ are multiplier variables, and $\beta>0$ is the penalty parameter.
In the algorithm and the later analysis, we introduce some additional notation.
For ease of notation, variables $\AB$, $\BB$, $\SB$, and $\DB$ are sometimes referred to as $\xB$, where $\xB=\big(\vecto(\AB);\vecto(\BB);\vecto(\SB);\vecto(\DB)\big)$.
Similarly, $\yB=\big(\yp;\yq;\vecto(\yd)\big)$.
With slight abuse of notation, we use $\lag(\AB,\BB,\SB,\DB,\yp,\yq,\yd,\beta)$ and $\lag(\xB,\yB,\beta)$ interchangeably.
By the definition of $\Omega_{r,k}(\pB,\qB)$, we have $0\le\DB\le\max\{\|\pB\|_\infty,\|\qB\|_\infty\}<1$.
Therefore, $\xB$ lies in a compact domain $\XM$.
Based on $\xB$, the equality constraints in $\Omega_{r,k}(\pB,\qB)$ can be rewritten as a vector function $\cB:\XM\to\zeroB^{m+n+mn}$ with the $u$\textsuperscript{th} entry
\begin{equation*}
	c_u(\xB)=\begin{cases}
		&\sum_{j=0}^{n-1}\sum_{l=0}^{r-1}A_{lk}B_{jk}+S_{lj}-p_u,\text{ if }0\le u<m\\
		&\sum_{i=0}^{m-1}\sum_{l=0}^{r-1}A_{ik}B_{u-m,l}+S_{i,u-m}-q_{u-m},\text{ if }m\le u<m+n\\
		&\sum_{l=0}^{r-1}A_{(u-m-n)\quo n,l}B_{(u-m-n)\rem n,l}+S_{(u-m-n)\quo n,(u-m-n)\rem n}-D_{(u-m-n)\quo n,(u-m-n)\rem n}, \text{ otherwise,}
	\end{cases}
\end{equation*}
where $\quo$ and $\rem$ denote the integer division and modulo operation respectively.
We further denote
\begin{equation*}
	h(\xB)=\lambda\|\SB\|_1+\ia(\AB)+\ib(\BB)+\id(\DB).
\end{equation*}
The pseudocode of the proposed inexact ALM is demonstrated in Algorithm \ref{alg:ialm}.
The high-level intuition is that we construct a series of strongly-convex and smooth \subproblems{}, each of which is solved inexactly by the block coordinate descent (BCD) in Algorithm \ref{alg:bcd}.
Such approach is guaranteed by the following proposition.
The proof is provided in the appendix.
\begin{proposition}
	Given $\yB$ and $\beta$, let $G(\xB)=\lag(\xB,\yB,\beta)+L(\yB,\beta)\|\xB-\bar{\xB}\|^2$ where
	\begin{equation}\label{eq:smoothness}
		L(\yB,\beta)=\sqrt{2r}\|\CB\|_F+\sqrt{2r}(m\sqrt{n}+n\sqrt{m}+mn)\|\yB\|+\beta L_c,
	\end{equation}
	with
	\begin{equation}
		\begin{aligned}
			B_u&=\max_{\xB\in\XM}\max\{|c_u(\xB)|,\|\nabla c_u(\xB)\|\},\\
			L_c&=\sum_{u=0}^{m-1}\sqrt{2nr}B_u+\sum_{u=m}^{m+n-1}\sqrt{2mr}B_u+\sum_{u=m+n}^{m+n+mn-1}\sqrt{2r}B_u+\sum_{u=0}^{m+n+mn-1}B_u^2.
		\end{aligned}
	\end{equation}
	Then, $G(\xB)$ is $3L(\yB,\beta)$-smooth and $L(\yB,\beta)$-strongly convex.
\end{proposition}

%bar{L}

\begin{algorithm}[ht]
	\caption{Inexact augmented Lagrangian method\label{alg:ialm}}
	\begin{algorithmic}[1]
		\State {\textbf{Input:}} $\epsilon$, $\beta_0>0$, $\sigma>1$, $w_0$, and $T$.
		\State {\textbf{Output:}} $\xB_T$.
		\State {\textbf{Initialization:}} $\xB_0\in\XM$, $\yB_0=\zeroB$.
		\For{$t=0$, $1$, $\dots$, $T-1$}
		\State Calculate $\beta_t=\beta_0\sigma^t$ and $L_t=L(\yB_t,\beta_t)$ as (\ref{eq:smoothness}).
		\State $\xB_{0,t}=\xB_t$.
		\For{$s=0$, $1$, $\dots$}
		\State Let $G_{s,t}(\cdot)=\lag(\cdot,\yB_t,\beta_t)+L_t\|\cdot-\xB_{s,t}\|^2$.
		\State $\xB_{s+1,t}=\bcd\big(G_{s,t}, h,\xB_{s,t}, L_t,\frac{\epsilon}{4}\big)$.
		\If{$2L(\yB_t,\beta_t)\|\xB_{s+1,t}-\xB_{s,t}\|\le\frac{\epsilon}{2}$}
		\State $\xB_{t+1}=\xB_{s+1,t}$.
		\State \textbf{Break.}
		\EndIf
		\EndFor
		\State $\yB_{t+1}=\yB_t+w_t\cB\big(\xB_{t}\big)$ where $w_t=w_0\min\{1,\frac{\log^2 2\|\cB(\xB_{1})\|}{(t+1)\log^2(t+2)\|\cB(\xB_{t+1})\|}\}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

\paragraph{BCD.}
Each BCD iteration updates one randomly selected matrix using the partial gradient of $G(\cdot)$.
Other three matrices are fixed.
Note that all BCD iterations admit closed-form solutions, since the indicator functions and the $\ell_1$ norm regularizer are \emph{proximal-friendly}.
%For example, if $\AB$ is to be updated at the $\tau$\textsuperscript{th} iteration,

\begin{algorithm}[ht]
	\caption{Block coordinate descent method: $\bcd(G, h, \xB_0, L, \delta)$\label{alg:bcd}}
	\begin{algorithmic}[1]
		\State {\textbf{Input:}} $\xB_0\in\XM$, smoothness $L$, and stationary tolerance $\delta$.
		\For{$\tau=0,1,\dots$}
		\State Choose $i_\tau\in\{0,1,2,3\}$ with probability $\frac{1}{4}$.
		\If{$i_\tau=0$}
		\State $\AB_{\tau+1}=\argmin_\AB\langle\nabla_\AB G(\xB_\tau),\AB\rangle+\frac{L}{2}\|\AB-\AB_\tau\|^2_F+\ia(\AB)$.
		\State $\BB_{\tau+1}=\BB_\tau$, $\SB_{\tau+1}=\SB_{\tau}$, and $\DB_{\tau+1}=\DB_\tau$.
		\ElsIf{$i_\tau=1$}
		\State $\BB_{\tau+1}=\argmin_\BB\langle\nabla_\BB G(\xB_\tau),\AB\rangle+\frac{L}{2}\|\BB-\BB_\tau\|^2_F+\ib(\BB)$.
		\State $\AB_{\tau+1}=\AB_\tau$, $\SB_{\tau+1}=\SB_{\tau}$, and $\DB_{\tau+1}=\DB_\tau$.
		\ElsIf{$i_\tau=2$}
		\State $\SB_{\tau+1}=\argmin_\SB\langle\nabla_\SB G(\xB_\tau),\SB\rangle+\frac{L}{2}\|\SB-\SB_\tau\|^2_F+\lambda\|\SB\|_1$.
		\State $\AB_{\tau+1}=\AB_\tau$, $\BB_{\tau+1}=\BB_{\tau}$, and $\DB_{\tau+1}=\DB_\tau$.
		\Else
		\State $\DB_{\tau+1}=\argmin_\DB\langle\nabla_\DB G(\xB_\tau),\DB\rangle+\frac{L}{2}\|\DB-\DB_\tau\|^2_F+\id(\DB)$.
		\State $\AB_{\tau+1}=\AB_\tau$, $\BB_{\tau+1}=\BB_{\tau}$, and $\SB_{\tau+1}=\SB_\tau$.
		\EndIf
		\If{$\dist\big(-\nabla G(\xB_{\tau+1}),\partial h(\xB_{\tau+1})\big)\le\delta$}
		\State \textbf{Return} $\xB_{\tau+1}=\big(\vecto(\AB_{\tau+1});\vecto(\BB_{\tau+1});\vecto(\SB_{\tau+1});\vecto(\DB_{\tau+1})\big)$
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}


\subsection{Complexity Analysis}
We first bound the number of BCD iterations that is required to reach a stationary point of (\ref{eq:problem_alm}).
The computational cost for each BCD iteration is then analyzed.
Finally, we obtain the overall complexity of Algorithm \ref{alg:ialm}.
For simplicity, we assume $m\le n$ without loss of generality in this subsection.
Detailed proofs are provided in the appendix.

\paragraph{Number of BCD iterations.}
Following the literature \citep{sahin2019inexact,li2021rate}, we analyze the complexity for reaching a first-order stationary point which is defined as follows.
\begin{definition}
	A pair $(\xB,\yB)$ is called an $\epsilon$-KKT point to (\ref{eq:problem_alm}) \citep{sahin2019inexact,li2021rate} if
	\begin{equation}
		\sqrt{\sum_{u=0}^{m+n+mn}c_u(\xB)^2}\le\epsilon,
	\end{equation}
	and
	\begin{equation}
		\dist\big(-\nabla_\xB \lag(\xB,\yB,\beta),\partial h(\xB)\big)\le\epsilon,
	\end{equation}
	hold,
	where the distance function between a vector $\aB$ and a set $\BM$ is defined as $\dist(\aB,\BM)=\min_{\bB\in\BM}\|\aB-\bB\|$.
\end{definition}
The main convergence result is summarized in the following theorem.
\begin{theorem}
	Algorithm \ref{alg:ialm} needs $T=\OM(\log\frac{1}{\epsilon})$ outer loops to produce an $\epsilon$-KKT solution of (\ref{eq:problem_alm}) and the total number of BCD iterations is $\OM\Big(\frac{1}{\epsilon^3}(\log\frac{1}{\epsilon})^2\Big)$.
\end{theorem}

\paragraph{Per-iteration complexity.}
The cost matrix $\CB$ is often low-rank \citep{scetbon2021low}, which can be exploited to accelerate the computation of BCD iterations.
Under suitable assumptions, the per-iteration complexity for each BCD iteration is $\OM(nr^2)$, which is stated in the following proposition.
\begin{proposition}
	When the following assumptions hold,
	\begin{enumerate}
		\item $\|\SB_\tau\|_0\le k'$ for all $\tau$ where $Tk'=\OM(nr)$,
		\item and $r\ge\rank(\CB)$,
	\end{enumerate}
	the per-iteration complexity for each BCD iteration is $\OM(nr^2)$ by exploiting the low-rank structure of $\CB$ in evaluating the partial gradients.
\end{proposition}
The first assumption is mild by choosing a moderately large $\lambda$.

The number of iterations is the same as the Sinkhorn method in terms of $\epsilon$ up to logarithm factors.
Therefore, if $r\ll \sqrt{m}$, Algorithm \ref{alg:ialm} is more efficient than Sinkhorn method.
%Note that we only need to explicitly calculate entries $D_{ij}$ if $S_{ij}<0$.
